HALOS: Hallucination-free Organ Segmentation after Organ Resection Surgery

The wide range of research in deep learning-based medical image segmentation pushed the boundaries in a multitude of applications. A clinically relevant problem that received less attention is the handling of scans with irregular anatomy, e.g., after organ resection. State-of-the-art segmentation models often lead to organ hallucinations, i.e., false-positive predictions of organs, which cannot be alleviated by oversampling or post-processing. Motivated by the increasing need to develop robust deep learning models, we propose HALOS for abdominal organ segmentation in MR images that handles cases after organ resection surgery. To this end, we combine missing organ classification and multi-organ segmentation tasks into a multi-task model, yielding a classification-assisted segmentation pipeline. The segmentation network learns to incorporate knowledge about organ existence via feature fusion modules. Extensive experiments on a small labeled test set and large-scale UK Biobank data demonstrate the effectiveness of our approach in terms of higher segmentation Dice scores and near-to-zero false positive prediction rate.

==> tables/ablation_UKB.tex <==
\begin{table*}
\footnotesize
\setlength{\tabcolsep}{4.6pt} % Reduce white-space between columns, SHOULD BE SET AFTER TABLE IS FINISHED
\caption{Comparison of our method with baselines (nnUnet, baseline Unet, oversampling, post-processing, Dice loss, multi-task paper)}
%0.453 \interval{0.072} 
\begin{tabular}{l c c c c c c}
    \toprule
    Method & FP & TN & TP & FN & FPR & bacc\\
    \midrule
    baseline Unet & $83.6$ & $268.4$ & $540.2$ & $62.8$  &$0.259$&  \\
    
    \addlinespace[0.3em]
    
    multi-task & $68.6$ & $283.4$ & $538.2$& $61.8$& $0.1949$ & $0.8269$ \\

  \addlinespace[0.3em]
  
     %baseline Unet + FF (GT) & & & & & &  \\

  %\addlinespace[0.3em]
  
 %   baseline Unet + FF (clf) & & & & & &  \\

  %\addlinespace[0.3em] 
  \midrule
  
   multi-task + FF (GT) & $2$& $350$ & $564.8$ & $35.2$ & $0.005682$ &  $0.9329$\\ 

  \addlinespace[0.3em]
  
  multi-task + FF (clf) & $11$ & $341$ & $541.8$ & $58.2$ & $0.03125$ &  $0.9329$\\

    \bottomrule
\end{tabular}

\label{tab:ablation_ukb}
\end{table*}


==> tables/ablation_segmentation.tex <==
\begin{table*}
\footnotesize
\setlength{\tabcolsep}{4.6pt} % Reduce white-space between columns, SHOULD BE SET AFTER TABLE IS FINISHED
\caption{Comparison of our method with baselines (nnUnet, baseline Unet, oversampling, post-processing, Dice loss, multi-task paper)}
%0.453 \interval{0.072} 
\begin{tabular}{l c c c c c c c c}
    \toprule
    Method & Mean Dice & liver & spleen & r kidney & l kidney & pancreas & gallbladder & FPR\\

    \midrule
    baseline Unet & $0.814$ & $0.934$ & $0.887$ & $0.900$ & $0.895$ & $0.651$ & $0.618$ & $0.267$ \\
    
    \addlinespace[0.3em]
    
  
    %baseline Unet + FF (GT) & & & & & & & \\

  %\addlinespace[0.3em]
   % using a separate classifier, e.g. DenseNet
    %baseline Unet + FF (clf) & & & & & & & \\

  %\addlinespace[0.3em] 

  multi-task & $0.821$ & $0.930$ & $0.880$ & $0.897$ & $0.887$ & $0.651$ & $0.682$ & $0.167$ \\

  \addlinespace[0.3em]
  
  \midrule
  
  
  multi-task + FF (GT) & $0.842$ & $0.935$ & $0.893$ & $0.898$ & $0.894$ & $0.646$ & $0.783$ & $0$\\
    \addlinespace[0.3em]

 multi-task + FF (clf) & $0.839$ & $0.935$ & $0.892$ & $0.898$ & $0.894$ & $0.644$ & $0.770$ & $0$\\


    \bottomrule
\end{tabular}

\label{tab:ablation_seg}
\end{table*}

